A Study of Nucleon Spin Struture from Quantum Chromodynamics

I present an introduction to the field of Quantum Chromodynamics (QCD) with emphasis on nucleon spin structure and perturbative methods. After a somewhat comprehensive overview of perturbative QCD, including the systematics of renormalization, I introduce deeply-inelastic scattering and deeply-virtual Compton scattering along with the nonperturbative distribution functions appearing in these processes. I show how these processes can be used to extract the distribution of longitudinal spin of nucleons, and briefly discuss the complications associated with transverse spin components. There are five appendices which accompany this work, discussing topics ranging from canonical field quantization to dimensional regularization to the structure of several important Lie groups. These appendices are meant to give the reader a certain basic understanding of some of the mathematical details underlying the main text, as well as provide a useful reference. This work was submitted in a slightly different form to the University of Maryland at College Park in partial completion of the requirements for a doctor of philosophy in physics, received August 2000.

==> abstract.tex <==
Quantum Chromodynamics (QCD) is thought to be the 
correct microscopic theory of the strong force.  
Composed only of eight colored gluons and
thirty-six colored quarks, its dynamics are
believed to generate the observed hadronic spectrum of
more than a thousand particles and account for many of their 
interactions - from the formation of nuclei to the rate
at which a $\rho$-meson decays.  Unfortunately, its predictions
are often beyond the reach of of our current understanding of 
quantum field theory.  Although the theory is perturbative
at high energy, the phenomenon of confinement makes direct
QCD calculations of physical observables quite intractable.

Through a process called factorization, one systematically 
separates the soft, incalculable physics from the 
perturbative high-energy physics.  The soft physics is then
grouped into matrix elements which can be measured in 
experiment.  Once fixed, these matrix elements can 
be used to predict the outcome of other experiments.  This
process allows one to indirectly test the validity of 
QCD in the perturbative regime.  Moreover, the matrix
elements themselves are of interest.  Acting as a window to
the nonperturbative physics of QCD, these objects allow us to link the 
quark and gluon degrees of freedom of the microscopic
theory to macroscopic observables such as hadron momentum
and spin.

This thesis presents a study of how these ideas can 
be used to understand the origins of nucleon spin.
Beginning with a general overview of QCD as a quantum field theory
in Chapter 1, we then move on to study inclusive 
Deeply-Inelastic Scattering
(DIS) in Chapter 2.  Inclusive DIS presents one of the earliest examples
of a factorizable process.  The soft physics relevant
to this process
is related to parton probability distributions, and provided
some of the first evidence that protons have nontrivial
internal structure.  We discuss the one-loop corrections to this
amplitude, the definitions and interpretations of the distribution
functions, and a proof that the hard and soft physics can be 
consistently separated at high energy to all orders in the QCD coupling.

The original research presented here concerns Deeply-Virtual Compton
Scattering (DVCS), a process closely related to DIS.  The special kinematics
of DVCS allow one to measure new hadronic parton distributions.
As explained in Chapter 3, these distributions contain information on
the origins of nucleon spin that DIS cannot provide.  We calculate
the one-loop coefficient functions of these new
distributions as they appear in DVCS and show that the soft physics
inherent to this process can be separated from the 
hard at this order.  Armed with the methods of 
Chapter 2, we then argue that this property persists to all
orders in the strong coupling.  Using our 
result, we calculate an operator product expansion 
for the product of two electromagnetic currents that is valid 
for a certain class of off-diagonal matrix elements.  This 
constitutes a generalization of the expansion first considered by 
Wilson in 1969, which has been used extensively over the past
thirty years.

Chapter 4 is devoted to the complications associated with 
transversely polarized DIS.  We discuss the special circumstances
that arise here due to the introduction of a 
transverse direction.  In particular, the gauge-invariance
of QCD demands that these effects be inseparable from
multiparton correlations within the nucleon.  Among other
things, this fact complicates the scale evolution of the relevant 
distributions.  We show that these complications are removed
at the one-loop level by taking the limit of large $N_c$.
Although this simplification has been known for several years, 
its origins have remained a mystery.  Our new approach to the
calculation allows us to directly
understand these origins.  We discuss the possibility
of similar simplifications at the higher loop level and for other
important distributions.
